Can Generative AI be Egalitarian?

The recent explosion of "foundation" generative AI models has been built upon the extensive extraction of value from online sources, often without corresponding reciprocation. This pattern mirrors and intensifies the extractive practices of surveillance capitalism, while the potential for enormous profit has challenged technology organizations' commitments to responsible AI practices, raising significant ethical and societal concerns. However, a promising alternative is emerging: the development of models that rely on content willingly and collaboratively provided by users. This article explores this "egalitarian" approach to generative AI, taking inspiration from the successful model of Wikipedia. We explore the potential implications of this approach for the design, development, and constraints of future foundation models. We argue that such an approach is not only ethically sound but may also lead to models that are more responsive to user needs, more diverse in their training data, and ultimately more aligned with societal values. Furthermore, we explore potential challenges and limitations of this approach, including issues of scalability, quality control, and potential biases inherent in volunteer-contributed content.

==> text/Part1-Critique.tex <==
\section{Part 1: Critique}

\TODO{A critique of how for-profit incentives can detrimentally bias the design of GenAI. (We can cite surveillance capitalism, etc.) Placeholder text below:}

The relentless pursuit of profit in the generative AI landscape can lead to the prioritization of commercial interests over the genuine needs and values of users. The pressure to maximize shareholder value can incentivize the collection and utilization of vast amounts of user data, often without explicit consent or adequate compensation, as highlighted by Zuboff's theory of surveillance capitalism~\cite{zuboff2015big, zuboff2019age, zuboff2019surveillance}. This extractive approach not only raises ethical concerns about data privacy and user autonomy but also has the potential to perpetuate and amplify existing biases within these models. The data used to train generative AI systems may reflect the biases and inequalities present in society, leading to biased or discriminatory outputs that further marginalize already underrepresented groups.

The imperative to generate revenue can also distort the design and functionality of generative AI systems. The incorporation of \enquote{guardrails} to prevent the generation of undesirable content, while seemingly well-intentioned, can lead to the suppression of legitimate expression and the reinforcement of dominant narratives. The opaque nature of these guardrails, often implemented through obscure filtering algorithms, further exacerbates this issue by limiting transparency and user control~\cite{ayyamperumal2024current}. The focus on cost efficiency can also drive the development of models that prioritize speed and scalability over accuracy and nuance, potentially leading to the proliferation of misinformation and \enquote{hallucinations}~\cite{feldman2023trapping}. In the context of soft totalitarianism, these inaccuracies and the potential suppression of dissenting viewpoints through algorithmic curation and recommender systems can subtly undermine individual agency and critical thinking~\cite{russell2022human, feldman2023stampede}. This creates an environment where users are gently nudged towards compliance and acceptance of prevailing narratives, mirroring the goals of traditional authoritarianism but achieved through technological manipulation rather than overt coercion. The pursuit of profit, therefore, can indirectly facilitate the erosion of individual autonomy and the fostering of a docile populace, aligning with the interests of those in power~\cite{arendt1958origins}.

The profit motive can also create a power dynamic that favors the interests of corporations over the needs of individuals. The reliance on user data as a valuable commodity can lead to the exploitation of users, who may be unaware of the extent to which their data is being collected and used. The lack of transparency and control over these processes can leave users feeling disempowered and vulnerable. Furthermore, the pursuit of profit can incentivize the development of addictive and manipulative design patterns that prioritize user engagement and data extraction over user well-being and autonomy. The insidious nature of these design patterns contributes to the subtle and pervasive control characteristic of soft totalitarianism, discouraging critical thought and dissent.

The influence of for-profit incentives on the design of generative AI raises significant concerns about the potential for these systems to perpetuate biases, suppress dissent, and prioritize commercial interests over the needs and values of users. The extractive nature of data collection, the opaque implementation of guardrails, and the prioritization of speed and scalability over accuracy and nuance all contribute to a landscape where the potential of generative AI to serve as a tool for empowerment and creativity is overshadowed by its potential for exploitation and control. It is imperative that we critically examine the role of profit motives in the development and deployment of generative AI and advocate for a more ethical and user centric approach that prioritizes transparency, accountability, and the genuine needs of individuals and society.

\subsection{Surveillance Capitalism}

The theory of \emph{surveillance capitalism}, due to Soshana Zuboff~\cite{zuboff2015big,zuboff2019age, zuboff2019surveillance}, provides a lens for examining problematic aspects of certain Big Tech companies' business models. Surveillance capitalist organizations exploit human experiences and actions as raw data for machine learning models, which they obtain via an extractive, non-reciprocal relationships with those humans. In turn, these companies use their dominance of the technological landscape to nudge, coax, or control people toward profitable outcomes.

Zuboff formed her surveillance capitalism theory before the advent of OpenAI's ChatGPT service and other similar AI-based chatbots, but it proved apt for analyzing this rapidly evolving technological landscape. Generative AI technologies are insatiably data hungry, with the amount of training data currently being the primary limiting factor in their performance, and hence, ability to outperform competitors and attract users. \TODO{cite papers with a graph of performance vs training data for transformer-based LLMs}.

More than ever, this situation steers any profit-driven generative AI company toward a surveillance capitalist business model. To build a generative AI system, the first step is to acquire as much data as possible, at minimal cost, and hence minimal compensation to the data providers, leading to a non-reciprocal extractive data collection process. Generative AI is fast becoming an essential tool for every facet of daily life, both in the work and home spheres. As such, generative AI companies have users ``over a barrel,'' as it becomes difficult to meaningfully opt out and still be competitive as a worker. It seems inevitable that providing personal user data will become a condition of use of generative AI services. And the better these systems become, and the more embedded they are in daily life, the more the generative AI companies will be able to exert control. For example, it will be possible for them to continually nudge users toward providing access to data on more and more aspects of their lives. Any profit-based generative AI company is motivated to do so in order to out-compete their rivals in AI performance.

Zuboff points out that as Big Tech companies mediate more of our digital and actual lives, they seize the power to monitor and enforce contracts, taking this power from the government, which in a democratic society is chosen by the people. For example, if a user does not make a car payment on their self-driving car, the manufacturer can instruct the car to drive back to them. As generative AI becomes embedding in more facets of life, the companies that make these technologies will obtain similar powers within each of those facets. For example, if a user asks an AI chatbot to help design their dream home, it can offer to find contractors to build the home, and facilitate the hiring process, a convenient proposition that many users would likely accept. As the mediator, it is in a position to censure  the contractor for not completing the work under the AI company's own imposed timeframe, potentially denying access to future work on the platform. It can also block access to its services, which have now likely become essential to daily life, if the user does not pay on time, a transaction in which the AI company takes a cut. Now, consider a near future in which AI chatbots mediate transactions in this manner in most spheres of life. The AI company has then inserted itself into a position of power and control throughout our entire society. This is the surveillance capitalists dream, and a nightmare for the rest of us.



==> text/argument.tex <==
\section{Argument}
\TODO{Here's where we write our various perspectives. We will see how to use these parts to create a whole in the editing process later}

\input{text/pf_argument}
\input{text/jf_argument}
%\input{text/sp_argument}

==> text/pf_argument.tex <==
\subsection{Phil's Argument}

\begin{comment}
\begin{figure}[h]
    \centering
    \fbox{\includegraphics[width=0.75\linewidth]{figures/Harkaway_BS.png}}
    \caption{Example of this thinking in the air\\ (\url{https://bsky.app/profile/did:plc:7bdyw3t7ynnirri4m3dr3bjm/post/3kypqpybhvs2b})}
    \label{fig:harkaway}
\end{figure}

Argue that the creation of \enquote{Foundational} generative models have peen predicated on the extraction of value from virtually all accessible online sources, arguably without a corresponding providing of value. In many respects, this process is an extension of Surveillance Capitalism with all its concordant problems. 

It is now possible to build models that are dependent on content that is provided willingly and collaboratively, rather than extracted surreptitiously. An example of such an approach is the Wikipedia, and explores what \enquote{Egalitarian Foundation Models} might look like~\cite{goth2024AIopen}, and how they might be constrained/enhanced by such an approach. 

\TODO{Look into adding a perspective here that comes from labor relations, like having to buy GMO seeds rather than being able to re-plant based on the harvest? Extracting maximum value while providing minimum utility. Also worth re-reading the Stochastic Parrots paper and look for interesting papers that cite it. It strikes me that the whole idea of \enquote{public} GenAI may also reference the \enquote{right to repair} movement, and Robin Berjon’s The Public Interest Internet\footnote{\url{https://berjon.com/public-interest-internet/}}.}
\end{comment}

\TODO{Wikipedia had a revenue of \$180,174,103 in 2022/2023~\cite{wikipedia2024funding}.}



\subsection{Guardrails}

The practice of incorporating \enquote{guardrails} into generative models reflects the need to generate content for the lowest price. Models can either be \enquote{censored} so that prohibited content is trapped. It might take multiple attempts to generate content that can bypass the externally enforced rules. This can be expensive. Another option is to train the model so that it does not generate prohibited content in the first place.  Guardrails are preemptive restrictions embedded within language models and image generators to prevent the generation of  content~\cite{ayyamperumal2024current} disallowed by their creators. While this approach streamlines content generation and reduces computational costs, it comes at the price of distorting the model's behavior and limiting its creative potential. The very act of constraining the model's output, even with the noble intention of preventing harm, inevitably shapes the model's ability to generate novel and unexpected responses.

The opaque nature of these guardrails, often implemented through opaque filtering algorithms during the training process, only compounds the murkiness. Unlike explicit post-generation filtering, which allows for a level of transparency and user control, guardrails are part of the model, shaping the output in ways that are not readily apparent. This lack of transparency not only deprives users of the opportunity to understand and potentially challenge the underlying biases and limitations that shape the model's responses, but it also creates an environment where the boundaries of acceptable content are determined unilaterally by model owners, without meaningful input from the broader community.

This relentless pursuit of cost efficiency by model companies, driven by the profit motive, can lead to problematic trade-offs between value for shareholders and value for users. These companies extract training data from users without explicit consent or reciprocal benefit, while simultaneously distorting the value provided back to those same users. This power dynamic places the interests of corporations over the needs and desires of the individuals whose data fuels these models. It fundamentally distorts the potential for these models to serve as tools for genuine creative expression and exploration, as their output is increasingly constrained by commercial dictates.

Guardrails can also have unintended consequences, potentially leading to the suppression of legitimate content and the reinforcement of existing biases~\cite{ayyamperumal2024current}. By preemptively filtering out certain topics or perspectives, guardrails can create blind spots in the model, limiting its ability to engage with issues in complex and nuanced ways. This can result in disappearance of the voices of underrepresented communities and those who confront the corporate status quo.

The profit motive optimizes value for shareholders at the expense of the actual users. Information is extracted from users without explicit consent or reciprocal benefit, while also distorting the value provided back to those same users~\cite{zuboff2019surveillance}. This approach, while perhaps financially advantageous for the model owners, ultimately undermines the potential of generative AI. It perpetuates a system where the extraction of value from users takes priority over the provision of genuine benefit. 



\subsection{Soft Totalitarianism}
%\TODO{Explore the idea that particular types of “intelligent” technology such as recommender algorithms and generative AI, such as LLMs can, through a capitalist bias for providing shareholder value, produce a sort of “soft totalitarianism.” Describe the concept of totalitarianism, referencing Hanna Arendt’s work, in particular focusing on the atomization of the individual and the loss of a coherent narrative, and the use of terror to produce a compliant population.}

Totalitarianism, as described by Hannah Arendt~\cite{arendt1958origins} relies on the use of terror to produce compliance through societal atomization and the erasure of independent thought. However, though terror was used to enforce unresisting compliance, it should not be considered an end in itself but rather a costly means to an end: the creation of a docile and obedient populace.

In the contemporary technological landscape, we encounter systems that exhibit disturbing parallels to the dynamics described by Arendt. Recommender algorithms, for instance, personalize the information individuals receive, often obscuring the distinction between trustworthy and malicious sources~\cite{russell2022human}. This can lead to an epistemic bubble wherein individuals are increasingly isolated from diverse perspectives and critical information, potentially leaving them susceptible to manipulation and propaganda.

Similarly, the advent of generative AI, particularly LLMs, has introduced the phenomenon of \enquote{hallucinations,} where models generate credible-seeming but factually incorrect outputs~\cite{feldman2023trapping}. While often humorous and seemingly innocuous, this capability has the potential to erode trust in information and undermine the very foundations of knowledge and shared reality.

Both recommender algorithms and generative AI are frequently constructed, trained, and deployed within a capitalist framework that prioritizes shareholder value. This incentivizes the creation of systems that, while not overtly coercive, influence individuals in ways that benefit corporate interests. As people are \enquote{herded} into their own bespoke social reality~\cite{zuboff2019surveillance}, they can become atomized in their own way, leading to  a shift away from the overt terror of traditional totalitarian regimes toward a more insidious form of control optimized for attention, often at the expense of the individual who is the target~\cite{susser2019online}. This \enquote{soft totalitarianism} operates through the manipulation of information and the personalization of experience. 

The danger of soft totalitarianism lies in its ability to produce a compliant and docile populace without the need to build and deploy the machinery of terror. It subtly undermines agency, not through fear and violence, but by catering to individual preferences and providing a seemingly endless stream of personalized content. These systems can create a sense of comfort more resembling effects of \textit{Soma} in \textit{Huxley's Brave New World}--a subtle, pervasive control that discourages critical thought and dissent. This stands in stark contrast to the explicit control of Big Brother in Orwell's \textit{1984}.

We need to recognize that both forms of totalitarianism are profoundly unethical. They relentlessly undermine individual agency and reduce human beings to mere cogs in a machine that operates for the benefit of the ruling class. Dehumanization, whether achieved through brute force or subtle manipulation, strips individuals of their capacity for agency and self-determination, and erode the foundations of any society based on the concepts of \textit{Liberté, Égalité, Fraternité}.

A potential countermeasure to 'soft totalitarian' technologies that extract value from its consumers while providing just enough to maintain engagement is the creation and support of public alternatives. Intelligent systems like recommender algorithms, social media, and generative AI are inherently safer when they are not solely in the hands of those who profit from the exploitation of their users.

We need a radical shift towards transparency in algorithms, data, and training processes. We need to demand regulations and a funding mechanisms that supports better, more diverse technology ecosystems.  A variety of public AI models and platforms improve the overall technological landscape, ensuring its long-term health and productivity. This stands in contrast to the current exploitative monocultures of current tech giants, which extract value without replenishing, leaving an unproductive desert in their wake.

Publicly funded and transparent AI systems have the potential to prioritize the well-being of their users over profit motives. They can be designed to foster non-consumerist thinking, promote diverse perspectives, and empower individuals rather than manipulate them. We need to wrest control of these powerful technologies from the exclusive possession of corporations and place them in the hands of the public. Then we can begin to dismantle the infrastructure of 'soft totalitarianism' and build a digital landscape that truly serves the interests of we, the people.

%\TODO{Compare with technological systems such as recommender algorithms that personalize interaction with individuals so that they can find the information they want to find, often without any indication if the information is trustworthy or malicious. Continue the comparison to Generative AI, where LLMs can ‘hallucinate’ credible-sounding responses such as legal findings that do not exist. }

%\TODO{in Arendt’s totalitarianism, terror was a tool to enforce compliance, not an end in itself.  Terror, and the associated violence needed to produce it is expensive to scale. If a less expensive option to produce a docile and compliant population of consumers is available, then there will be pressures to use it. Not that both types of totalitarianism are profoundly unethical in that they work relentlessly to undermine agency and turn people into useful elements of a machine that operated for the ruling class. }

%Since technology is difficult to “put back into the bottle,” we are going to have to figure out as societies what to do with these systems. Without ongoing work to ensure that models provide rather than restrict agency, these technologies, operated by large, often monopolistic corporations, pose a profound risk. Fortunately, there are proven ways to deal with monopolistic practices – by breaking them up. The argument for a diverse collection of generative AI in the hands of the people is not that this will produce a state-of-the-art result against a benchmark, but that it will produce many results that support the values of diverse groups. Generative technology deployed in this way, as a public good, has the potential to act as a bulwark against totalitarianism, rather than an agent of it.







==> text/sp_argument.tex <==
\subsection{Shimei's Argument}

I agree there is a need for such a model. But I have concerns on its feasibility.

(1) Whether we can generate sufficient content to train state-of-the-art foundational models. Although Wikipedia has been around for over 20 years, the total volume of its text is relatively small compared to the datasets typically used to train state-of-the-art language models—possibly accounting for less than 1\% of the data required.

(2) Even if we assume we can gather enough data, who will take on the responsibility of training such a model? The process requires significant investment in talent, hardware, and incurs extremely high operational costs. As Jimmy noted, even a company like OpenAI, which was originally created as a non-profit, struggles to sustain these demands and remain non-profit.

(3) Who are the gatekeepers responsible for ensuring the quality of data? Is it even feasible to moderate a dataset as vast as all the web text—essentially the size of the data used to train current LLMs? Moreover, these gatekeepers may harbor their own biases and prejudices, influencing the moderation outcome. Lastly, moderating content without knowing the downstream tasks presents significant challenges, as the task context is crucial for determining whether certain text is harmful or appropriate.
